DeepRacing: Parameterized Trajectories for Autonomous Racing

We consider the challenging problem of high speed autonomous racing in a realistic Formula One environment. DeepRacing is a novel end-to-end framework, and a virtual testbed for training and evaluating algorithms for autonomous racing. The virtual testbed is implemented using the realistic F1 series of video games, developed by Codemasters, which many Formula One drivers use for training. This virtual testbed is released under an open-source license both as a standalone C++ API and as a binding to the popular Robot Operating System 2 (ROS2) framework. This open-source API allows anyone to use the high fidelity physics and photo-realistic capabilities of the F1 game as a simulator, and without hacking any game engine code. We use this framework to evaluate several neural network methodologies for autonomous racing. Specifically, we consider several fully end-to-end models that directly predict steering and acceleration commands for an autonomous race car as well as a model that predicts a list of waypoints to follow in the car's local coordinate system, with the task of selecting a steering/throttle angle left to a classical control algorithm. We also present a novel method of autonomous racing by training a deep neural network to predict a parameterized representation of a trajectory rather than a list of waypoints. We evaluate these models performance in our open-source simulator and show that trajectory prediction far outperforms end-to-end driving. Additionally, we show that open-loop performance for an end-to-end model, i.e. root-mean-square error for a model's predicted control values, does not necessarily correlate with increased driving performance in the closed-loop sense, i.e. actual ability to race around a track. Finally, we show that our proposed model of parameterized trajectory prediction outperforms both end-to-end control and waypoint prediction.

==> sections/qual_exam_cover_page/coverpage.tex <==
Pages 2 and onward of this document are intended to satisfy the requirement for my PhD Qualification Exam as earlier proposed to you, the Qualification Exam Committee.  This work has also been submitted for review to be included in the Journal of Machine Learning Research (JMLR).  Additionally, I have selected 3 papers that I have read in detail related to this work and am prepared to answer questions about them during my examination:

\begin{enumerate}
    \item ~\bibentry{pilotnet}
    \item ~\bibentry{auto-encoder}
    \item ~\bibentry{LSTM-occupancy-grid}
\end{enumerate}

\newpage
